Fast Inexact Bilevel Optimization for Analytical Deep Image Priors

The analytical deep image prior (ADP) introduced by Dittmer et al. (2020) establishes a link between deep image priors and classical regularization theory via bilevel optimization. While this is an elegant construction, it involves expensive computations if the lower-level problem is to be solved accurately. To overcome this issue, we propose to use adaptive inexact bilevel optimization to solve ADP problems. We discuss an extension of a recent inexact bilevel method called the method of adaptive inexact descent of Salehi et al.(2024) to an infinite-dimensional setting required by the ADP framework. In our numerical experiments we demonstrate that the computational speed-up achieved by adaptive inexact bilevel optimization allows one to use ADP on larger-scale problems than in the previous literature, e.g. in deblurring of 2D color images.

==> Figs/coloured/semi-blind/motion_Gaussian_1/regularizer_1.0_1e-06_motion_blur/data/2 <==
xÌL>9‡V¸r•86.O¸']7Hª]¸gâL>N¬¹CƒÂ8€ÖT¸j›8t¹wñL>þG¹õ§8±‰V¸à!Å8Z¹
ãL>‡Íb¸«°7ˆ°S¸68:M]¸–ÌL>ËÌL>¼6e¸˜(*8N`¸\æ*7~Ëk¸½äL>X6 ¹€ò×8†Ïf¸ó)#8!¹HõL>Ø÷#¹é)8J§d¸Oh×8Þ#¹ÊåL>ê]u¸2_(7ĝb¸'°/8Ìôn¸ûÌL>ÇÌL>ém`¸`#8ÐW¸W7šfg¸õãL>0ƒ¹Î7Ì8'ƒ\¸Øp8Œ·¹5óL>'¹m¤8/]¸DÄÌ8ÿ¹çãL>rŽh¸½?7ƄY¸Ã|"8b¸«ÌL>
